FairBranch: Mitigating Bias Transfer in Fair Multi-task Learning

The generalisation capacity of Multi-Task Learning (MTL) suffers when unrelated tasks negatively impact each other by updating shared parameters with conflicting gradients. This is known as negative transfer and leads to a drop in MTL accuracy compared to single-task learning (STL). Lately, there has been a growing focus on the fairness of MTL models, requiring the optimization of both accuracy and fairness for individual tasks. Analogously to negative transfer for accuracy, task-specific fairness considerations might adversely affect the fairness of other tasks when there is a conflict of fairness loss gradients between the jointly learned tasks - we refer to this as Bias Transfer. To address both negative- and bias-transfer in MTL, we propose a novel method called FairBranch, which branches the MTL model by assessing the similarity of learned parameters, thereby grouping related tasks to alleviate negative transfer. Moreover, it incorporates fairness loss gradient conflict correction between adjoining task-group branches to address bias transfer within these task groups. Our experiments on tabular and visual MTL problems show that FairBranch outperforms state-of-the-art MTLs on both fairness and accuracy.

==> ablation.tex <==
\subsection*{Ablation Study}
To select the best $\tau$ we validate our model over the values: $(0.6,0.7,0.8)$. Intuitively lower values would mean loosely grouped tasks, while very high values would result in more single task branches, increasing the number of parameters. We also checked for relative percentage of parameters that \our{} needs for a given $\tau$, compared to total parameters required for training $T$ \verb|STL|s (each task with a dedicated \verb|STL|). We depict our findings in table~\ref{tab.ablation}. 
%We found that for tabular data $\tau$=$0.7$ produced the best trade-off, while surprisingly requiring less parameters compared to that with $\tau$=$0.5$. A similar behaviour is also observed in visual data, where even though $\tau$=$0.6$ produced the best trade-off,  $\tau$=$0.8$ led to less parameters compared with  $0.4$. %Upon investigation, we found that at times with lower values of $\tau$ as the model finds groups with loose attachment, it passes comparatively less effective knowledge to the parameters below. Eventually, this hurts the model as the branches become more dissimilar, requiring the model to find more standalone branches as it goes deep into the shared parameters.   
\begin{table}[htb!]
%\vspace{-0.1in}
\centering
\small % Reduce font size
\caption{\small Ablation Study with Varying $\tau$ on Validation Data. RP: Relative Parameters Compared to Training STL for each Task, ARA (Accuracy), and ARF (Fairness).}\label{tab.ablation}
\setlength{\tabcolsep}{5pt} % Reduce column spacing
\begin{tabular}{|c|l|c c|c c|}
\hline
\textbf{$\boldsymbol{\tau}$} & \textbf{Metric} & \multicolumn{2}{c|}{\textbf{ACS-PUMS}} & \multicolumn{2}{c|}{\textbf{CelebA}}\\
& &\textbf{18-19} & \textbf{19-21} & \textbf{gen} & \textbf{age} \\
%\hline
%  \multirow{3}{*}{0.4} & ARA & 0.97 & 1.06 & 1.06 & 1.04\\
% & \multirow{2}{*}{ARF \begin{tabular}[c]{@{}|c@{}}EP\\EO\end{tabular}} & 1.05 & 0.96 & 1.86 & 6.73\\
% &  & 1.08 & 0.95 & 1.52 & 1.07\\
% & RP & 0.41 & 0.70 & 0.39 & 0.41 \\
% \hline
%\cline{2-6}
% \multirow{3}{*}{0.5} & ARA & 0.99 & 1.08 & 1.03 & 1.02\\
% & \multirow{2}{*}{ARF \begin{tabular}[c]{@{}|c@{}}EP\\EO\end{tabular}} & 1.07 & 0.93 & 2.88 & 2.30\\
% &  & 1.07 & 0.93 & 1.71 & 1.27\\
% & RP & 0.55 & 0.63 & 1.30 & 0.39\\
\hline
\multirow{3}{*}{0.6} & ARA & 0.98 & 1.03& 1.03 &  1.01\\
& \multirow{2}{*}{ARF \begin{tabular}[c]{@{}|c@{}}EP\\EO\end{tabular}} &0.95 & 1.06& 1.38 & 3.07\\
& &0.97 & 1.07 & 1.13 & 1.20\\
& RP & 0.55 & 0.41 & 0.37 & 0.39\\
\hline
%\cline{2-6}
\multirow{3}{*}{0.7} & ARA & 1.00& 1.07& 1.03 & 1.03\\
& \multirow{2}{*}{ARF \begin{tabular}[c]{@{}|c@{}}EP\\EO\end{tabular}} &0.96 & 1.00 & 2.41& 3.83\\
&  & 0.97 & 0.99& 1.79 & 1.27\\
& RP & 0.41 & 0.41 & 0.35 & 0.48\\
\hline
\multirow{3}{*}{0.8} & ARA & 0.99 & 1.07 & 0.97 & 1.04\\
& \multirow{2}{*}{ARF \begin{tabular}[c]{@{}|c@{}}EP\\EO\end{tabular}} & 1.01 & 0.93 & 1.74 & 5.05\\
&  & 1.02 & 0.93 & 1.56 & 1.29\\
& RP &0.73 & 0.41& 0.29 & 0.40\\
%\hline
\hline
\end{tabular}
\end{table}
